Radiative neutrino masses and the Cohen-Kaplan-Nelson bound

Recently, an increasing interest in UV/IR mixing phenomena has drawn attention to the range of validity of standard quantum field theory. Here we explore the consequences of such a limited range of validity in the context of radiative models for neutrino mass generation. We adopt an argument first published by Cohen, Kaplan and Nelson that gravity implies both UV and IR cutoffs, apply it to the loop integrals describing radiative corrections, and demonstrate that this effect has significant consequences for the parameter space of radiative neutrino mass models.

==> Makefile <==
all: build/paper.pdf

build/paper.pdf: content/01_introduction.tex plots

build/paper.pdf: FORCE | build
	TEXINPUTS="$(call translate,build:)" \
	BIBINPUTS=build: \
	max_print_line=1048576 \
	latexmk \
	  --lualatex \
	  --output-directory=build \
	  --interaction=nonstopmode \
	  --halt-on-error \
	paper.tex

	cp build/paper.pdf paper.pdf
	rm -rf build

build:
	mkdir -p build

plots: plotFile.py
	mkdir -p plots
	python3 plotFile.py

clean:
	rm -rf plots
	rm -rf build
	rm paper.pdf

FORCE:

.PHONY: all clean FORCE


==> content/01_introduction.tex <==


